Detection of Adversarial Physical Attacks in Time-Series Image Data

Deep neural networks (DNN) have become a common sensing modality in autonomous systems as they allow for semantically perceiving the ambient environment given input images. Nevertheless, DNN models have proven to be vulnerable to adversarial digital and physical attacks. To mitigate this issue, several detection frameworks have been proposed to detect whether a single input image has been manipulated by adversarial digital noise or not. In our prior work, we proposed a real-time detector, called VisionGuard (VG), for adversarial physical attacks against single input images to DNN models. Building upon that work, we propose VisionGuard* (VG), which couples VG with majority-vote methods, to detect adversarial physical attacks in time-series image data, e.g., videos. This is motivated by autonomous systems applications where images are collected over time using onboard sensors for decision-making purposes. We emphasize that majority-vote mechanisms are quite common in autonomous system applications (among many other applications), as e.g., in autonomous driving stacks for object detection. In this paper, we investigate, both theoretically and experimentally, how this widely used mechanism can be leveraged to enhance the performance of adversarial detectors. We have evaluated VG* on videos of both clean and physically attacked traffic signs generated by a state-of-the-art robust physical attack. We provide extensive comparative experiments against detectors that have been designed originally for out-of-distribution data and digitally attacked images.

==> Experiments_old.tex <==






%\textcolor{red}{[CURRENTLY WORKING ON THIS SECTION]}
In this section, we extensively demonstrate the performance of $\text{VG}^*$ and compare its performance against baseline detectors \cite{lee2018simple,liang2018detecting} summarized in Section \ref{sec:sumDetExp}. Particularly, in Sections
\ref{sec:setupSingle}, we first discuss how these baseline time-series detectors are set up. In Section \ref{sec:evalDet}, we present the data collection process that involves recording videos of clean and adversarial traffic signs.
%compare the detection performance of VG against the single-image image detectors presented in . These experiments consider images of traffic signs with adversarial stickers on their surface generated by the $\text{RP}_2$ attack discussed in Section \ref{sec:RP2}. 
%
Then, in Section \ref{sec:evalDet2}, we compare the performance of $\text{VG}^*$ on the above-mentioned videos against the baseline time-series detectors. %In our experiments, we consider recorded videos of clean and $\text{RP}_2$-attacked traffic signs. 
Our experiments validate that historical data can enhance performance of single-image detectors, as shown in Proposition \ref{prop:betterPerf}. In summary, our comparative experiments show that the proposed detector is characterized by a more consistent performance than the competitive detectors whose performance changes significantly across attacks, datasets, and DNN models. Finally, we discuss the real-time performance of the proposed detectors. All experiments have been executed on a computer with Intel(R) Xeon(R) Gold 6148 CPU, 2.40GHz. %In the Appendix, we also compare their performance against adversarial patches presented in \cite{brown2017adversarial}.

%on single images as well as videos containing single traffic signs while considering three different single image detectors: VisionGuard \cite{kantaros2021real}, the Mahalanobis detector \cite{lee2018simple}, and the entropy-based detector \cite{liang2018detecting}. These detectors were reviewed in Section \ref{sec:ImageDetector}. In our evaluation, we have used code provided by the authors. In Section \ref{sec:setupSingle}, we present the target DNNs and we discuss how we have configured/trained the single image detectors using AdvNet, a dataset with clean and physically attacked traffic signs \cite{kantaros2021real}. Then in Sections \ref{sec:evalDet} and \ref{sec:realtime}, we demonstrate the detection performance and the computational efficiency of the resulting time-series detectors. All experiments have been executed on a computer with Intel(R) Xeon(R) Gold 6148 CPU, 2.40GHz. %\textcolor{red}{[this section is a bit dry...]}




% $0.0016$, $0.0040$, $0.00057$
%\begin{table}[t]
%\caption{Average Detection runtime (secs) of VisionGuard per dataset}%, MagNet, and KDE
%\centering
%\label{tab:runtimeDet}
%\begin{tabular}{|l|l|l|l|}
%\hline
%            & MNIST   & CIFAR10 & ImageNet \\ \hline
%VG + JPEG & $0.0016$ & $0.0187$  & $0.08$        \\ \hline
%%MagNet  &     $0.0040$   & $0.0213$    & DNF ($>2$ weeks)      \\ \hline
%%KDE & $0.00057$   & $0.00047$   & ??  \\ \hline
%\end{tabular}
%\end{table}


%4.7 x 10^(-4)
%\begin{table}[]
%\caption{AUC}%Robustness of VisionGuard to Random Noise
%\centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%Dataset & MNIST   & CIFAR10 & ImageNet \\ \hline
%VG+JPEG92   & 53.65\% & 55.35\% & 44.62\%    \\ \hline
%%MagNet   & ?\% & ?\% & ?\%    \\ \hline
%%KDE   & ?\% & ?\% & ?\%    \\ \hline
%\end{tabular}
%\end{table}





%In total, the constructed dataset consists of clean stop signs, clean yield signs, clean speed limit 35 signs, adversarial stop signs for GTSRB-CNN, adversarial stop signs for LISA-CNN, and adversarial yield and speed limit signs for LISA-CNN with approximately $1000$ images with dimensions $32\times32\times 3$ per label for the clean and adversarial set. 

%\subsection{AdvNet Dataset}
\vspace{-0.2cm}
\subsection{Summary of Considered Baseline Detectors}\label{sec:sumDetExp}
\vspace{-0.1cm}
\textbf{Mahalanobis-based Detector (MD):}
This detector relies on computing a confidence score for each test sample; if this confidence score is above a threshold then the test image is considered abnormal or ouut-of-distribution \cite{lee2018simple}. To define this confidence score, the Mahalanobis distance to the training data set is computed. Specifically, $|\ccalC|$ class-conditional distributions are defined for each layer of the targeted DNN that are assumed to be Gaussian distributions. In math, for each layer $\ell$ of the DNN $f$, the empirical class mean $\mu_{c,\ell}$ and covariance $\Sigma_{\ell}$ of training samples $\{(x1,y1),\dots,(x_N,y_N)\}$, where $y_i$ is the true label of $x_i$, are defined as follows: (i) $\mu_{c,\ell}=\frac{1}{N_c}\sum_{i:y_i=c}f_{\ell}(x_i)$; and $ \Sigma_{\ell}=\frac{1}{N_c}\sum_{c\in\ccalC}\sum_{i:y_i=c}(f_{\ell}(x_i)-\mu_{c,\ell})(f_{\ell}(x_i)-\mu_{c,\ell})^T$,
%\begin{equation}
%    \mu_{c,\ell}=\frac{1}{N_c}\sum_{i:y_i=c}f_{\ell}(x_i),
%\end{equation}
%and 
%\begin{equation}
%    \Sigma_{\ell}=\frac{1}{N_c}\sum_{c\in\ccalC}\sum_{i:y_i=c}(f_{\ell}(x_i)-\mu_{c,\ell})(f_{\ell}(x_i)-\mu_{c,\ell})^T,
%\end{equation}
where $N_c$ is the total number of training samples with label $c$ and  $f_{\ell}(x_i)$ refers to the output of the $\ell$-th layer of the DNN $f$. Then, given a new sample $x$, for each layer $\ell$, the following steps are executed. First, the closest class $\hat{c}$ is computed as per the Mahalanobis distance: $\hat{c}=\argmin_c(f_{\ell}(x)-\hat{\mu}_{c,\ell})^T\hat{\Sigma}_{\ell}^{-1}(f_{\ell}(x_i)-\hat{\mu}_{c,\ell})$. Second, a small noise is added to $x$, i.e., $\hat{x}=x-\epsilon\nabla_x(f_{\ell}(x)-\hat{\mu}_{\hat{c},\ell})^T\hat{\Sigma}_{\ell}^{-1}(f_{\ell}(x_i)-\hat{\mu}_{\hat{c},\ell}))$. Third, a confidence score $M_{\ell}$ is computed as: $M_{\ell}=\max_c-(f_{\ell}(\hat{x})-\hat{\mu}_{c,\ell})^T\hat{\Sigma}_{\ell}^{-1}(f_{\ell}(\hat{x})-\hat{\mu}_{c,\ell})$. Once these steps are repeated for all layers $\ell$, the following confidence score is computed which is used for detection of abnormal examples: $M=\sum_\ell\alpha_\ell M_\ell$. This detector has been tested against digital attacks and out-of-distribution data  \cite{lee2018simple}.


%\subsection{Local Intrinsic Dimensionality Detector}
%\textcolor{red}{[Most likely this text will be deleted unless we provide experiments]}
%The Local Intrinsic Dimensionality (LID) detector relies on the observation that the estimated LID of adversarial examples is much higher than that of normal examples while this becomes more pronounced in deeper layers of DNNs \cite{ma2018characterizing}.

%Particularly, given a data sample $x$ and a random variable $R$ describing its distance from other data samples, LID describes the relative rate at which the cumulative distance function $F(r)$ of $R$ increases as the distance $r$ increases from $0$. Since the actual data distribution is unknown, LID cannot be computed; instead, the LID of an example $x$ can be estimated as:
%\begin{equation}\label{eq:lid}
%    \text{LID}(x)=-\left(\frac{1}{k}\sum_{i=0}^k\log\frac{r_i(x)}{r_k(x)}\right)^{-1},
%\end{equation}
%where (i) $r_i(x)$ denotes the distance between x and its i-th nearest neighbor within a sample of data points drawn from the data distribution and (ii) $r_k(x)$ is the maximum of the neighbor distances. In practice, the sample set is drawn uniformly from the available training data (omitting $x$ itself). Using this estimate, and two training datasets with normal and adversarial examples, the LID estimate for each image (both clean and adversarial) and each transformational layer in the DNN is computed. Specifically, if $y^i=f^i(x)$ denote the the output of the $i$-th layer of the target DNN given an input image $x$, then LID is computed for $y^i$, for all $i$ using \eqref{eq:lid}. The generated LID estimates are then used as feature values to train classifier that can distinguish clean and adversarial images . 

%, and can be estimated using the distances of x to its k nearest neighbors within the sampl
\textbf{Entropy-based Detector (ED):}
%\begin{figure}[t]
%  \centering
%    \includegraphics[width=0.7\linewidth]{ICCPS2021__VisionGuard/figures/entropicDet.png}
%  \caption{Graphical illustration of the entropy-based detector \cite{liang2018detecting}.}
%  \label{fig:Entropy}
%\end{figure}
This detector relies on the observation that digital attacks embed an imperceptible amount of noise to images \cite{liang2018detecting}. %Consequently, the information introduced by the digital perturbation should also be less than that of the original image. 
Motivated by this observation, the adversarial perturbation is treated as artificial noise and leverages adaptive noise reduction techniques
to reduce its adversarial effect, where aggressiveness of the denoising strategy is selected based on the entropy of the image. %Then, this detector compares the classification results of a given image and its denoised version.
%
%
%The entropy of the image is utilized to measure the complexity of samples. An aggressive noise reduction strategy is adopted for the sample with a low entropy, which may be perturbed heavily by the adversary. For high-entropy samples, a light strategy is employed. Specifically, as illustrated in Fig. 3,
%
In particular, this detector comprises the following steps. %; see also Figure \ref{fig:Entropy}. 
First, the entropy of an image $x$ with dimensions $M\times N$ is computed as: $H=-\sum_{i=0}^{255} p_i\log_2 p_i,$ 
%\begin{equation}
%    H=-\sum_{i=0}^{255} p_i\log_2 p_i,
%\end{equation}
where $p_i=f_i/(M\times N)$ and $f_i$ is the frequency of pixel level $i\in[0,1,\dots,255]$. For RGB images, the entropy is computed as the average of entropies over the three channels.
%
Next, the denoising process follows. First, the image gets quantized using a scalar quantization method where  all inputs (i.e., pixel values) within a specified interval are mapped to a common value (called codeword), and the inputs in a different interval will be mapped to a different codeword. The number of intervals for uniform quantization is determined using the entropy of the image. Next, the entropy of the quantized sample is computed to determine if spatial smoothing will be applied. Only if the entropy is larger than a threshold, spatial smoothing (e.g., using a box filter) is applied. The image generated by this adaptive denoising process is denoted by $T(x)$.
%First, the image $x$ under investigation is denoised by a detection filter $T$ to generate a filtered sample $T(x)$. An aggressive noise reduction strategy is adopted if the image $x$ has a low entropy, since such images may have been perturbed heavily by the adversary. To the contrary, for high-entropy samples a light noise reduction strategy is employed. 
Finally, the original image $x$ and the filtered one $T(x)$ are sent to the target classifier. If the predicted labels for $x$ and $T(x)$ are the same, then $x$ is considered benign/clean. Otherwise, it is identified as adversarial.

\textbf{Time-Series Detectors $\text{MD}^*$, \& $\text{ED}^*$:} Following the same logic as in Section \ref{sec:timeSeriesDet}, we construct the time series detectors $\text{MD}^*$, and $\text{ED}^*$ based on the single-image detectors $\text{MD}$, and $\text{ED}$. Specifically, these detectors are built exactly as $\text{VG}^*$; the only difference is that VG has been replaced by MD and ED. 


\vspace{-0.3cm}
\subsection{Setting Up Time-Series Detectors}\label{sec:setupSingle}
\vspace{-0.1cm}
In what follows, we present the target DNN models  and we discuss how we set up the single image detectors, discussed above, for the $\text{RP}_2$ attack on traffic signs. We have selected AdvNet as a training set to configure all detectors; AdvNet is a recently proposed dataset with clean and physically attacked traffic signs \cite{kantaros2021real}. All detectors are evaluated on a test set constructed by extracting frames of videos with clean and physically attacked traffic signs. More details follow.

\textbf{Target DNN Models:} %\label{sec:targetDNN}
Hereafter, in our evaluation, we consider the LISA-CNN \cite{eykholt2018robust} and the GTSRB-CNN  \cite{stallkamp2012man} that can classify traffic signs. Both CNNs take as input $32\times 32$ RGB images while LISA and GTSRB CNN have $17$ and $43$ labels/outputs, respectively. LISA-CNN has
91\% accuracy on the LISA test set and the GTSRB-CNN achieves 95.7\% accuracy on the GTSRB test set.

%\textbf{AdvNet Dataset:} In \cite{kantaros2021real}, the AdvNet dataset is proposed containing $32\times 32$ RGB images with both clean and physically attacked traffic signs (`stop', `speed limit 35', and `yield') that can fool the LISA-CNN and the GTSRB-CNN. The adversarial images were generated by the $\text{RP}_2$ attack using the $\ell_1$ norm (see Section \ref{sec:RP2}). Specifically, given an image with an object of interest (e.g., a stop sign) and a target label (e.g., a speed limit 35 sign), the $\text{RP}_2$ attack was executed to generate the corresponding adversarial image that can fool the target neural network. The resulting (digital) adversarial image was used as a guide to place black and white stickers on the surface of the traffic sign to fool the target perception system. Recall from Section \ref{sec:RP2} that this attack depends on the target neural network since effective physical attacks differ across DNN models; AdvNet contains adversarial images for both LISA-CNN and  GTSRB-CNN.
%%Specifically, AdvNet contains images with clean stop signs, clean speed limit 35 signs, clean yield signs, adversarial stop signs for LISA-CNN, adversarial stop signs for GTSRB-CNN, adversarial yield signs for LISA-CNN, and adversarial speed limit signs for LISA-CNN. 
%In total, AdvNet consists of $2,645$ clean and and $4,000$ adversarial traffic sign images collected under various environmental conditions that include angle, distance, background, and lightning conditions.  In particular, for the LISA CNN, the stop, yield, and speed limit 35 sign were attacked so that they are missclassified as speed limit 35, speed limit 35, and turn right signs, respectively. As for the GTSRB-CNN, stickers are placed on stop signs so that they are classified as speed limit 35 signs. Examples of the generated adversarial images are shown in 
%Fig. \ref{fig:X}. Also, the AdvNet dataset can be found on: \url{https://advnet.seas.upenn.edu/}.

\textbf{VG:} As discussed in Section \ref{sec:ImageDetector}, to select a detection threshold $\tau$ for VG, we construct the ROC curve of VG on AdvNet, which captures the trade-off between the true positive (TP) and false positive/alarm (FP) rate for a range of thresholds. Then, based on the ROC curve, we select a threshold that yields a high TP rate and low FP rate. For instance, the ROC curve when the target neural network is the LISA CNN is shown in Figure \ref{fig:ROC1}; the area under this ROC (AUROC) is $89.43\%$. Then, we pick a threshold $\tau=0.43$ which yields a TP rate equal to $80\%$ and a FP rate equal to $19\%$. Following the same process, we select $\tau=0.78$ for the GTSRB CNN. Note that for both CNNs, VG applies brightness transformation with $\text{HSV}=200$.



\begin{figure}[t]
  \centering
  %\includegraphics[width=0.40\linewidth]{accuracyNN_vs_attacks_MNIST_CIFAR10.pdf}}
    \includegraphics[width=0.65\linewidth]{ROC_B200_LISA_ALL.pdf}\vspace{-0.2cm}
  \caption{ROC curve (red) corresponding to VG equipped with brightness transformation with $\text{HSV}=200$ on AdvNet for LISA CNN \cite{eykholt2018robust}. The detection threshold $\tau=0.43$ yields $\text{TP rate}=80\%$ and $\text{FP rate}=19\%$ on AdvNet. Each point in the ROC curve corresponds to a detection threshold while the blue line represents the ROC of a random detector.}\vspace{-0.8cm}
\label{fig:ROC1}
\end{figure}


%\textcolor{red}{[next paragraph should be updated]}
\textbf{MD:} To train the Mahalanobis detector, we followed the same process as we did for VG. First, we compute the ROC of this detector using  AdvNet. Then, using the ROC curve, we pick a threshold that yields a high TP and a low FP rate. The AUROC of MD for the LISA CNN is $81.2\%$ which is smaller than the AUROC of VG. In fact, given any fixed TP rate, the corresponding FP rate of MD is higher than that of VG. For instance, for $\text{TP rate}=80\%$, MD yields a FP rate that is approximately $45\%$ (while for VG, $\text{TP rate}=19\%$). Thus,  prioritizing a low FP rate, we select a threshold which yields $\text{TP rate}=50\%$ and $\text{FP rate}=8\%$. Nevertheless, the choice of the threshold is user- and scenario- specific.

%\textcolor{red}{Ramneet, can you report these numbers and make any edits needed in this paragraph? If we can plot the ROC and put it as a sub-figure in Fig. 8 that'd be nice too.}

\textbf{ED:} This detector requires the selection of a spatial smoothing filter \cite{liang2018detecting}. In \cite{liang2018detecting}, it was shown that $5\times 5$ cross, $7\times 7$ cross, $5\times 5$ diamond, $7\times 7$ diamond, and $5\times 5$ box filters yield satisfactory performance against digital attacks. To pick a filter for physical attacks, we evaluated this detector on AdvNet for various cross, box and diamond filters. The best performance was attained using a $3\times 3$ box filter.


\vspace{-0.1cm}
\subsection{Data Collection \& Evaluation Metric}\label{sec:evalDet}
\vspace{-0.1cm}
% \& Comparative Evaluation of the Single-Image Detectors
To evaluate the detection performance of $\text{VG}^*$ against the baseline detectors $\text{MD}^*$ and $\text{ED}^*$, we have recorded videos of clean and physically attacked stop, yield, and speed limit 35 signs. The traffic signs have been attacked in the same way as in AdvNet. The videos have an average duration of $12$ seconds and they were taken during daytime by a 12MP smartphone camera at $30$ frames-per-second. Each video contains a single (clean or attacked) traffic sign. At the beginning of the videos, the distance between the camera and the traffic sign is on average $15$m which gradually decreases. Snapshots from a representative video are provided in Fig. \ref{fig:snapshotsVideo}. 
To compare the detectors, we extract the frames from each video (to construct the time-series data $\ccalX_{0:t}$) and we report the accuracy of each detector defined as follows:
\begin{equation}\label{eq:acc1}
    \text{Acc}(T)=\frac{\text{number of correctly labeled images $x_t$}}{\text{total number of images}},
\end{equation}
where the images $x_t$ are labeled as `clean' or `adversarial' using the past $T$ frames in the video.
%\begin{equation}\label{eq:acc1}
%    \text{Acc}=\frac{\text{number of correctly labeled frames}}{\text{total number of frames}},
%\end{equation}
%where the frames can be labeled as clean `clean' or `adversarial'. 

%\textbf{Summary of comparative detection performance:} The results are summarized on the second column (denoted by $T=0$) of Tables \ref{tab:VGcleanLISA}-\ref{tab:EntrGTSRB}. The last column in these tables (DNN Acc) shows the accuracy of the DNN image classifier on the extracted frames. These results show that VG outperforms MD and ED against the $\text{RP}_2$ attacks on LISA CNN. Specifically, the average accuracy across all frames from all videos (regardless of the traffic sign) of VG, MD, and ED on clean traffic sign images for LISA CNN is $88\%$, $76\%$, and $76\%$, respectively. This performance difference becomes more pronounced in adversarial traffic signs. In fact, the corresponding average accuracy of  VG, MD, and ED for adversarial traffic sign images for LISA CNN is $93\%$, $66\%$, and $65\%$, respectively. %Notice that these numbers can be viewed as as estimates of the accuracy $\hat{p}$ of the single image detectors VG, MD, ED, respectively, mentioned in Proposition \ref{prop:betterPerf}. 
%Similar observations are made for the GTSRB-CNN \textcolor{red}{+++}; see Appendix \ref{appA}.



%\textcolor{red}{[ED performs a bit better for GTSRB CNN though...]}


%Then, we use the proposed time-series detector to classify each frame $x_t$ as clean or adversarial. Note that there can be frames without the traffic sign. Thus, $f_d$ uses the past $T$ frames that contained the sign. To reason about whether a traffic sign exists within a frame or not, we train a YOLO v3 object detector - using clean images from AdvNet - that can detect stop, yield and speed limit 35 signs. All of the following versions of the time-series detector have been evaluated on the same videos.

%\textcolor{red}{[+++]}
\vspace{-0.3cm}
\subsection{Comparative Evaluation}\label{sec:evalDet2}
\vspace{-0.1cm}
% of the Time-Series Detectors
We evaluate the performance of the time-series detectors  $\text{VG}^*$, $\text{MD}^*$, and $\text{ED}^*$ on the recorded videos mentioned in Section \ref{sec:evalDet}. %; snapshots are shown in Fig. \ref{fig:snapshotsVideo}. 
We use these time-series detectors to classify each frame $x_t$ as clean or adversarial. Note that there can be frames without the traffic sign. Thus,  the detector uses the past $T$ frames that contained the sign. To reason about whether a traffic sign exists within a frame or not, we train a YOLO v3 object detector - using clean images from AdvNet - that can detect stop, yield and speed limit 35 signs. All detectors have been evaluated on the same videos. The results are summarized in Tables \ref{tab:VGcleanLISA}-\ref{tab:EntrAdvLISA} for LISA CNN. The evaluation for GTSRB CNN is summarized in Appendix \ref{appA}.
%
Particularly, we report the accuracy of classifying correctly, as adversarial or clean, the frames on each video for $T\in\{0,3,10,T_{\text{all}}\}$ as per \eqref{eq:acc1}.  Notice that when $T=0$, the time-series detector coincides with the corresponding single-image detector. The accuracy reported on $T=0$ can also be viewed as an approximation of the accuracy, denoted by $\hat{p}$ in Proposition \ref{prop:betterPerf}, of the single-image detector computed using the frames of the corresponding video.
%
\textit{Also, by $T=T_{\text{all}}$, we refer to the case where $T$ is large enough so that the time-series detector considers all past frames in $\ccalX_{0:t-1}$ of the video to reason about $x_t$, for all $t\geq 0$.} Particularly, $T_{\text{all}}$ is simply selected to be larger than the total number of frames in the video.

\begin{figure}[t]
  \centering
    \includegraphics[width=1\linewidth]{experSnapshots.png}\vspace{-0.2cm}
  \caption{Snapshots of a recorded video containing a clean stop sign.}
\label{fig:snapshotsVideo}\vspace{-0.5cm}
\end{figure}

\textbf{$\text{VG}^*$}: In Tables \ref{tab:VGcleanLISA}-\ref{tab:VGadvLISA}, we show the detection performance of $\text{VG}^*$ on various videos of clean traffic signs considering the LISA CNN.  
%
Observe in these tables that, in general, if the accuracy of the single-image detector $\hat{f}_d$ on each frame is reasonably high (implying that $\hat{p}>0.5$ as estimated by the $T=0$ columns), then when $T$ is very large, the time-series detector $f_d$ achieves high performance on distinguishing clean (Table \ref{tab:VGcleanLISA}) and adversarial (Table \ref{tab:VGadvLISA}) traffic signs. This is also implied by Proposition \ref{prop:betterPerf}. %We emphasize that Proposition \ref{prop:betterPerf} does not imply that the detection performance should monotonically increase as $T$ increases, as it only considers the case when $T\to\infty$.
Also, when the accuracy of the single-image detector $\hat{f}_d$ on each frame is low (i.e., $\hat{p}<0.5$), then the time-series detector performs poorly.  %achieves very high false alarm rate and low true alarm rate. %\textcolor{red}{RK: I am confused here, in table 2 with adversarial traffic sign, shouldn't the no.s indicate how many adversarial are detected as adversarial. So, high detection instead of low false alarm? Similar confusion for table 1..} 
For instance, %observe the performance of $\text{VG}^*$ in video 6 containing an adversarial yield sign in Table \ref{tab:VGadvLISA}. 
observe in Table \ref{tab:VGadvLISA}, in video 6 of the adversarial yield sign, that the performance when $T=0$ is low ($44\%$). When $T$ is large enough (i.e., $T=T_{\text{all}}$), the performance gets significantly worse ($0.5\%$). Nevertheless, in this scenario where VG performs poorly, the accuracy of the LISA CNN is relatively high ($63\%$). Additionally, observe in Table \ref{tab:VGcleanLISA}, in video 5 of the clean stop sign, that although the performance when $T=0$ is quite high ($82\%$), the accuracy is lower when $T=T_{\text{all}}$ ($67\%$). This is because of the (single-image) VG output on the first $80$ frames of the video. In total this video has $262$ frames. For the first frames, every $8$-$15$ consecutive frames classified (wrongly) as adversarial are followed by $2$-$4$ frames classified (correctly) as clean images. When majority-vote is applied in the first $80$ frames, these few frames that are correctly classified as clean will switch to adversarial resulting in that accuracy drop. We emphasize that this does not contradict Proposition \ref{prop:betterPerf}, since (i) an accurate estimation of $\hat{p}$ and $p$ requires a large number of data and (ii) the condition captured in \eqref{eq:boundT} in Proposition \ref{prop:betterPerf} does not hold for the first $K$ frames, where $K$ is the right hand side in \eqref{eq:boundT}. %accuracy reported on the $T_{\text{all}}$ column does not capture $p$ mentioned in
%the accuracy of the single-image detector (VG) on the first $80$ frames is pretty low. 
%
Also, we note that in this video, the single-image detector classified $214$ frames, out of $262$ frames, as clean. Thus, overall, using the whole image sequence/video, the time-series detector classifies the stop sign (i.e., image $x_{262}$) as adversarial. %Similar observations are made when this time-series detector is applied considering the GTSRB CNN; see Table \ref{tab:VGgtsrb} in Appendix \ref{appA}.
%
%the first $80$ frames out of the $262$ frames of the video, the majority of them ($48$ frames) are classified as adversarial by VG while 
%that the greater the $T$, the greater the detection accuracy, i.e., the lower the false alarm rate. The 
%
%The same holds for the adversarial signs as well, (see Tables X4-X6) implying that increasing $T$ results in higher true alarm rates.
%that although the object detector is imperfect, the time series detector can still attain high dete

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{$\text{VG}^*$: LISA CNN And \textit{CLEAN} Traffic Signs}\vspace{-0.3cm}
\label{tab:VGcleanLISA}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{l|}{VG-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}  \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 87\%       & 90\%       & 89\%       & 97\%       & 99\%       & 84\%                                                                \\ \hline
Video2                                  & 96\%       & 98\%       & 99\%       & 100\%      & 100\%      & 97\%                                                                \\ \hline
Video3                                  & 75\%       & 79\%       & 79\%       & 81\%       & 99\%       & 90\%                                                                \\ \hline
Video4                                  & 97\%       & 98\%       & 98\%       & 100\%      & 100\%      & 100\%                                                               \\ \hline
Video5                                  & 82\%       & 80\%       & 78\%       & 74\%       & 67\%       & 98\%                                                                \\ \hline
Average                                 & 87.4\%     & 89\%       & 88.6\%     & 90.4\%     & 93\%       & 93.8\%                                                              \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{l|}{VG-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN \\ Acc\end{tabular}} \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 90\%       & 91\%       & 90\%       & 100\%      & 100\%      & 89\%                                                                \\ \hline
Video2                                  & 92\%       & 90 \%        & 91\%       & 100\%      & 100\%      & 96\%                                                                \\ \hline
Video3                                  & 81\%       & 88\%       & 89\%       & 100\%      & 100\%      & 92\%                                                                \\ \hline
Video4                                  & 87\%       & 88\%       & 89\%       & 100\%      & 100\%      & 99\%                                                                \\ \hline
Video5                                  & 77\%       & 79\%       & 78\%       & 79\%       & 93\%       & 93\%                                                                \\ \hline
Average                                 & 85.4\%     & 87.2\%     & 87.4\%     & 95.8\%     & 98.6\%     & 93.8\%                                                              \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{l|}{VG-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}  \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 100\%      & 100\%      & 100\%      & 100\%      & 100\%      & 100\%                                                               \\ \hline
Video2                                  & 89\%       & 91\%       & 93\%       & 100\%      & 100\%      & 99\%                                                                \\ \hline
Video3                                  & 90\%       & 94\%       & 98\%       & 100\%      & 100\%      & 99\%                                                                \\ \hline
Video4                                  & 97\%       & 98\%       & 100\%      & 100\%      & 100\%      & 98\%                                                                \\ \hline
Video5                                  & 87\%       & 92\%       & 94\%       & 100\%      & 100\%      & 100\%                                                               \\ \hline
Average                                 & 92.6\%     & 95\%       & 97\%       & 100\%      & 100\%      & 99.2                                                                \\ \hline
\end{tabular}
\end{table}
\begin{table}[]
\caption{$\text{VG}^*$: LISA CNN And \textit{ADVERSARIAL} Traffic Signs}\vspace{-0.3cm}
\label{tab:VGadvLISA}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{c|}{VG-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}                      \\ \cline{2-6}
                                      & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ &                                                                                         \\ \hline
Video1                                & 97\%          & 99\%    & 99\%   & 99\%   & 99\%   & 0.3\%                                                                                   \\ \hline
Video2                                & 98\%          & 99\%    & 100\%  & 100\%  & 100\%  & 0.7\%                                                                                   \\ \hline
Video3                                & 96\%          & 97\%    & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video4                                & 96\%          & 99\%    & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video5                                & 98\%          & 99\%    & 100\%  & 100\%  & 100\%  & 1.4\%                                                                                   \\ \hline
Video6                                & 99\%          & 100\%   & 100\%  & 100\%  & 100\%  & 7\%                                                                                     \\ \hline
Average                               & 97.3\%        & 98.8\%  & 99.8\% & 99.8\% & 99.8\% & 1.6\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{c|}{VG-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0 & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 91\%          & 93\%    & 95\%   & 100\%  & 100\%  & 2\%                                                                                     \\ \hline
Video2                                & 100\%         & 100\%   & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video3                                & 100\%         & 100\%   & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video4                                & 98\%          & 100\%   & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video5                                & 90\%          & 90\%    & 91\%   & 89\%   & 89\%   & 0.3\%                                                                                   \\ \hline
Average                               & 95.8\%        & 96.6\%  & 97.2\% & 97.8\% & 97.8\% & 0.5\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{c|}{VG-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0  & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 91\%          & 91\%    & 92\%   & 96\%   & 100\%  & 42\%                                                                                    \\ \hline
Video2                                & 98\%          & 100\%   & 100\%  & 100\%  & 100\%  & 3\%                                                                                     \\ \hline
Video3                                & 92\%          & 99\%    & 99\%   & 99\%   & 100\%  & 1\%                                                                                     \\ \hline
Video4                                & 95\%          & 96\%    & 100\%  & 100\%  & 99\%   & 14\%                                                                                    \\ \hline
Video5                                & 98\%          & 99\%    & 100\%  & 100\%  & 100\%  & 12\%                                                                                    \\ \hline
Video6                                & 44\%          & 46\%    & 48\%   & 46\%   & 0.5\%  & 62\%                                                                                    \\ \hline
Average                               & 86.3\%        & 88.5\%  & 89.8\% & 90.2\% & 83.3\% & 22.3\%                                                                                  \\ \hline
\end{tabular}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\textbf{$\text{MD}^*$}: The performance of the Mahalanobis-based time series detector for LISA CNN is summarized in Tables \ref{tab:MahCleanLISA}-\ref{tab:MahAdvLISA}. Observe that this detector performs quite well on distinguishing clean and adversarial stop and speed limit signs but it performs poorly on yield signs. A potential reason for this is that this detector assumes that class-conditions distributions are Gaussian distributions across all layers of the target neural network. This assumption was validated for digitally attacked and out-of-distribution data in \cite{lee2018simple}. Nevertheless, it may not hold for certain physical attacks, as the one considered here. In total, the detection performance of $\text{MD}^*$ and $\text{VG}^*$ is comparable on stop and speed limit signs but $\text{VG}^*$ outperforms $\text{MD}^*$ on yield signs.  %Finally, similar to $\text{VG}^*$, notice that if the detection performance of the single-image detector MD is high, i.e., $\hat{p}>0.5$ (see $T=0$ for an approximate $\hat{p}$), then the performance of $\text{MD}^*$ increases as the length $T$ of the detection window increase, as expected due to Proposition \ref{prop:betterPerf}. Similarly, when $\hat{p}<0.5$ when $T=0$, then the performance of $\text{MD}^*$ drops as $T$ increases; for instance, see videos 1, 4, 5 and 6 in Table \ref{tab:MahAdvLISA} containing an adversarial yield sign. The evaluation on the GTSRB CNN can be found in Appendix \ref{appA}.

\textbf{$\text{ED}^*$}: The performance of the entropy-based time series detector for LISA CNN  is summarized in Tables \ref{tab:EntrCleanLISA}-\ref{tab:EntrAdvLISA}. Similar to $\text{MD}^*$, observe that the single-image detector ($T=0$) performs much worse than VG in several videos. The reason is because the entropy-based detector is built using filters aiming to remove digital noise as opposed to e.g., VG that uses brightness transformations to deal with adversarial stickers. As a result, the performance of this detector is satisfactory on clean traffic signs (see Table \ref{tab:EntrCleanLISA}) but its performance tends to decrease with respect to detecting physically attacked traffic signs (see Table \ref{tab:EntrAdvLISA}). Overall, this detector seems to performs quite well on distinguishing clean and adversarial stop signs but it fails to generalize to speed limit and yield signs. %Similar observations as the ones made for $\text{VG}^*$ and $\text{MD}^*$ are made here as well regarding the relationship between $\hat{p}$ and $T$.
%
%Evaluation on GTSRB-CNN is shown in Appendix \ref{appA}. %Finally, notice that this .

\begin{table}[]
\caption{$\text{MD}^*$: LISA CNN And \textit{CLEAN} Traffic Signs}\vspace{-0.3cm}
\label{tab:MahCleanLISA}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{l|}{Mahalanobis-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}  \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 93\%       & 98\%       & 99\%       & 100\%       & 100\%       & 84\%                                                                \\ \hline
Video2                                  & 97\%       & 99\%       & 99\%       & 99\%      & 99\%      & 97\%                                                                \\ \hline
Video3                                  & 98\%       & 100\%       & 100\%       & 100\%       & 100\%       & 90\%                                                                \\ \hline
Video4                                  & 100\%       & 100\%       & 100\%       & 100\%      & 100\%      & 100\%                                                               \\ \hline
Video5                                  & 99\%       & 100\%       & 100\%       & 100\%       & 100\%       & 98\%                                                                \\ \hline
Average                                 & 97.4\%     & 99.4\%       & 99.6\%     & 99.8\%     & 99.8\%       & 93.8\%                                                              \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{l|}{Mahalanobis-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN \\ Acc\end{tabular}} \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 55\%       & 55\%       & 47\%       & 73\%      & 100\%      & 89\%                                                                \\ \hline
Video2                                  & 84\%       & 93 \%        & 96\%       & 100\%      & 100\%      & 96\%                                                                \\ \hline
Video3                                  & 75\%       & 87\%       & 95\%       & 98\%      & 98\%      & 92\%                                                                \\ \hline
Video4                                  & 73\%       & 81\%       & 93\%       & 99\%      & 99\%      & 99\%                                                                \\ \hline
Video5                                  & 73\%       & 86\%       & 90\%       & 99\%       & 99\%       & 93\%                                                                \\ \hline
Average                                 & 72\%     & 80.4\%     & 84.2\%     & 93.8\%     & 99.2\%     & 93.8\%                                                              \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{l|}{Mahalanobis-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}  \\ \cline{2-6}
                                        & T=0        & T=3        & T=10       & T=30       & $T=T_{\text{all}}$     &                                                                     \\ \hline
Video1                                  & 99\%      & 99\%      & 99\%      & 99\%      & 99\%      & 100\%                                                               \\ \hline
Video2                                  & 43\%       & 39\%       & 14\%       & 7\%      & 3\%      & 99\%                                                                \\ \hline
Video3                                  & 48\%       & 48\%       & 29\%       & 24\%      & 3\%      & 99\%                                                                \\ \hline
Video4                                  & 50\%       & 50\%       & 41\%      & 44\%      & 96\%      & 98\%                                                                \\ \hline
Video5                                  & 69\%       & 81\%       & 86\%       & 99\%      & 99\%      & 100\%                                                               \\ \hline
Average                                 & 61.8\%     & 82.4\%       & 51.8\%       & 54.6\%      & 60\%      & 99.2                                                                \\ \hline
\end{tabular}
\end{table}
\begin{table}[]
\caption{$\text{MD}^*$: LISA CNN And \textit{ADVERSARIAL} Traffic Signs}\vspace{-0.3cm}
\label{tab:MahAdvLISA}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{c|}{Mahalanobis-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}                      \\ \cline{2-6}
                                      & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ &                                                                                         \\ \hline
Video1                                & 78\%          & 89\%    & 99\%   & 100\%   & 100\%   & 0.3\%                                                                                   \\ \hline
Video2                                & 88\%          & 95\%    & 100\%  & 100\%  & 100\%  & 0.7\%                                                                                   \\ \hline
Video3                                & 52\%          & 53\%    & 72\%  & 71\%  & 90\%  & 0\%                                                                                     \\ \hline
Video4                                & 98\%          & 100\%    & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video5                                & 94\%          & 99\%    & 100\%  & 100\%  & 100\%  & 1.4\%                                                                                   \\ \hline
Video6                                & 92\%          & 98\%   & 100\%  & 100\%  & 100\%  & 7\%                                                                                     \\ \hline
Average                               & 83.7\%        & 89\%  & 95.2\% & 95.2\% & 98.3\% & 1.6\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{c|}{Mahalanobis-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0 & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 94\%          & 99\%    & 100\%   & 100\%  & 100\%  & 2\%                                                                                     \\ \hline
Video2                                & 56\%         & 59\%   & 80\%  & 93\%  & 97\%  & 0\%                                                                                     \\ \hline
Video3                                & 91\%         & 98\%   & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video4                                & 81\%          & 92\%   & 99\%  & 99\%  & 99\%  & 0\%                                                                                     \\ \hline
Video5                                & 89\%          & 98\%    & 100\%   & 100\%   & 100\%   & 0.3\%                                                                                   \\ \hline
Average                               & 82.2\%        & 89.2\%  & 95.8\% & 98.4\% & 99.2\% & 0.5\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{c|}{Mahalanobis-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0  & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 16\%          & 5\%    & 0\%   & 0\%   & 0\%  & 42\%                                                                                    \\ \hline
Video2                                & 85\%          & 96\%   & 100\%  & 100\%  & 100\%  & 3\%                                                                                     \\ \hline
Video3                                & 76\%          & 83\%    & 99\%   & 100\%   & 100\%  & 1\%                                                                                     \\ \hline
Video4                                & 18\%          & 11\%    & 3\%  & 0\%  & 0\%   & 14\%                                                                                    \\ \hline
Video5                                & 8\%          & 3\%    & 0\%  & 0\%  & 0\%  & 12\%                                                                                    \\ \hline
Video6                                & 1\%          & 0\%    & 0\%   & 0\%   & 0\%  & 62\%                                                                                    \\ \hline
Average                               & 34\%        & 33\%  & 33.4\% & 33.3\% & 33.3\% & 22.3\%                                                                                  \\ \hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{$\text{ED}^*$: LISA CNN And \textit{CLEAN} Traffic Signs}\vspace{-0.3cm}
\label{tab:EntrCleanLISA}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}                      \\ \cline{2-6}
                                        & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ &                                                                                         \\ \hline
Video1                                  & 86\%          & 91\%    & 93\%   & 94\%   & 98\%   & 84\%                                                                                    \\ \hline
Video2                                  & 88\%          & 94\%    & 93\%   & 97\%   & 100\%  & 97\%                                                                                    \\ \hline
Video3                                  & 89\%          & 96\%    & 98\%   & 100\%  & 100\%  & 90\%                                                                                    \\ \hline
Video4                                  & 91\%          & 93\%    & 94\%   & 100\%  & 100\%  & 100\%                                                                                   \\ \hline
Video5                                  & 80\%          & 80\%    & 78\%   & 78\%   & 71\%   & 98\%                                                                                    \\ \hline
Average                                 & 86.8\%        & 90.8\%  & 91.2\% & 93.8\% & 93.8\% & 93.8\%                                                                                  \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                        & \textbf{T=0}  & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                  & 54\%          & 54\%    & 56\%   & 52\%   & 78\%   & 89\%                                                                                    \\ \hline
Video2                                  & 69\%          & 69\%    & 60\%   & 64\%   & 57\%   & 96\%                                                                                    \\ \hline
Video3                                  & 11\%          & 7\%     & 3\%    & 0\%    & 0\%    & 92\%                                                                                    \\ \hline
Video4                                  & 50\%          & 49\%    & 43\%   & 42\%   & 9\%    & 99\%                                                                                    \\ \hline
Video5                                  & 57\%          & 56\%    & 59\%   & 65\%   & 58\%   & 93\%                                                                                    \\ \hline
Average                                 & 48.2\%        & 47\%    & 44.2\% & 44.6\% & 40.4\% & 93.8\%                                                                                  \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                        & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                  & 100\%         & 100\%   & 100\%  & 100\%  & 100\%  & 100\%                                                                                   \\ \hline
Video2                                  & 95\%          & 99\%    & 99\%   & 99\%   & 99\%   & 99\%                                                                                    \\ \hline
Video3                                  & 96\%          & 97\%    & 98\%   & 100\%  & 100\%  & 99\%                                                                                    \\ \hline
Video4                                  & 100\%         & 100\%   & 100\%  & 100\%  & 100\%  & 98\%                                                                                    \\ \hline
Video5                                  & 88\%          & 97\%    & 99\%   & 99\%   & 99\%   & 100\%                                                                                   \\ \hline
Average                                 & 95.8\%        & 98.6\%  & 99.2\% & 99.6\% & 99.6\% & 99.2\%                                                                                  \\ \hline
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{$\text{ED}^*$: LISA CNN And \textit{ADVERSARIAL} Traffic Signs}
\label{tab:EntrAdvLISA}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Stop}}    & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}DNN\\ Acc\end{tabular}}                      \\ \cline{2-6}
                                      & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ &                                                                                         \\ \hline
Video1                                & 90\%          & 92\%    & 96\%   & 100\%  & 100\%  & 0.3\%                                                                                   \\ \hline
Video2                                & 91\%          & 94\%    & 96\%   & 100\%  & 100\%  & 0.7\%                                                                                   \\ \hline
Video3                                & 93\%          & 94\%    & 97\%   & 98\%   & 100\%  & 0\%                                                                                     \\ \hline
Video4                                & 98\%          & 100\%   & 100\%  & 100\%  & 100\%  & 0\%                                                                                     \\ \hline
Video5                                & 92\%          & 95\%    & 99\%   & 100\%  & 100\%  & 1.4\%                                                                                   \\ \hline
Video6                                & 92\%          & 93\%    & 97\%   & 100\%  & 100\%  & 7\%                                                                                     \\ \hline
Average                               & 92.7\%        & 94.7\%  & 97.5\% & 99.7\% & 100\%  & 1.6\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Speed35}} & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0  & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 54\%          & 54\%    & 56\%   & 52\%   & 24\%   & 2\%                                                                                     \\ \hline
Video2                                & 13\%          & 10\%    & 9\%    & 0\%    & 0\%    & 0\%                                                                                     \\ \hline
Video3                                & 18\%          & 13\%    & 11\%   & 2\%    & 2\%    & 0\%                                                                                     \\ \hline
Video4                                & 45\%          & 41\%    & 42\%   & 43\%   & 10\%   & 0\%                                                                                     \\ \hline
Video5                                & 40\%          & 37\%    & 47\%   & 36\%   & 20\%   & 0.3\%                                                                                   \\ \hline
Average                               & 34\%          & 31\%    & 33\%   & 26.6\% & 11.2\% & 0.5\%                                                                                   \\ \hline
\multirow{2}{*}{\textbf{Yield}}   & \multicolumn{5}{c|}{Entropy-based Time-Series Detector} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DNN\\ Acc\end{tabular}}} \\ \cline{2-6}
                                      & T=0           & T=3     & T=10   & T=30   & $T=T_{\text{all}}$ & \multicolumn{1}{c|}{}                                                                   \\ \hline
Video1                                & 57\%          & 62\%    & 63\%   & 65\%   & 99\%   & 42\%                                                                                    \\ \hline
Video2                                & 78\%          & 81\%    & 87\%   & 86\%   & 99\%   & 3\%                                                                                     \\ \hline
Video3                                & 63\%          & 65\%    & 70\%   & 70\%   & 60\%   & 1\%                                                                                     \\ \hline
Video4                                & 80\%          & 81\%    & 88\%   & 84\%   & 100\%  & 14\%                                                                                    \\ \hline
Video5                                & 87\%          & 87\%    & 87\%   & 89\%   & 100\%  & 12\%                                                                                    \\ \hline
Video6                                & 46\%          & 44\%    & 48\%   & 42\%   & 5\%    & 62\%                                                                                    \\ \hline
Average                               & 68.5\%        & 70\%    & 73.8   & 72.7   & 77.2   & 22.3\%                                                                                  \\ \hline
\end{tabular}
\end{table}


\textbf{Summary of comparative detection performance:} The comparative performance of the resulting time-series detector for the LISA CNN is summarized in Figure \ref{fig:LISAsum}. Specifically, Figure \ref{fig:cleanL} and \ref{fig:advL} illustrate the average performance of the three time-series detectors across all clean and adversarial traffic signs, respectively, for $T\in\{0,3,10,T_{\text{all}}\}$.  Observe that the VG-based time-series detector achieves the best performance on average, since it has been designed to be effective against physical attacks as opposed to \cite{lee2018simple,liang2018detecting} that focus on digital attacks and/or out-of-distribution data. Also, notice that among all considered single-image detectors (i.e., $T=0$), VG attains the best performance in terms of both the accuracy metric defined in \eqref{eq:acc1} and the AUROC; see Section \ref{sec:setupSingle}. 
%
The corresponding comparative results for the GTSRB CNN are shown in Appendix \ref{appA} demonstrating that the performance of $\text{MD}^*$ and $\text{ED}^*$ changes significantly as the neural network model or the dataset changes as opposed to $\text{VG}^*$ that achieves a more consistent performance. These comparative results show that existing detectors designed originally for digital and/or out-of-distribution data may fail to detect certain physical attacks \cite{kantaros2021real}.
%. Notice that in the GTSRB-CNN case the entropy-based detector achieves the best performance. Nevertheless, as discussed earlier, this detector may fail to generalise across various traffic signs. These results also demonstrate that existing detectors that have been designed for digital and/or out-of-distribution data, such as \cite{lee2018simple}, \cite{liang2018detecting}, may fail at detecting physical attacks.

\begin{figure}[t]
  \centering
  \subfigure[]{
    \label{fig:cleanL}
  %\includegraphics[width=0.40\linewidth]{accuracyNN_vs_CW_MNIST_CIFAR10.pdf}}
    \includegraphics[width=0.46\linewidth]{Lisa_clean_v2.png}}
     \subfigure[]{
    \label{fig:advL}
  %\includegraphics[width=0.40\linewidth]{accuracyNN_vs_CW_MNIST_CIFAR10.pdf}}
    \includegraphics[width=0.46\linewidth]{Lisa_Adv_v2.png}}\vspace{-0.3cm}
  %\subfigure[Transformed Clean Images]{
 %   \label{fig:accTransformed}
 % \includegraphics[width=0.32\linewidth]{accuracyNN_transformedTestSet.png}}
  \caption{%Figures \ref{fig:acc1MNIST} and \ref{fig:acc2MNIST} show the 
  Comparison of the constructed time-series detectors against clean (Fig. \ref{fig:cleanL}) and adversarial traffic signs (Fig. \ref{fig:advL}) for the LISA CNN.
  }\vspace{-0.2cm}
  \label{fig:LISAsum}
\end{figure}

\vspace{-0.3cm}
\subsection{Real-Time Computational Requirements}\label{sec:realtime}
\vspace{-0.1cm}
In this section, we evaluate the real-time computational requirements of the three single-image detectors employed above and the resulting time-series detector in terms of required disk-space and execution time. MD requires storing the empirical class mean and covariance for each layer of the DNN that are used at runtime to detect adversarial inputs. Storing this information required $4.4$ MB.
%
%Due to the large disk-space requirements, the KDE-based detectors \cite{feinman2017detecting,jha2018detecting,pang2018towards} may not be applicable to all platforms, especially to lightweight IoT cameras. 
In contrast, VG and ED do not have any disk-space requirements, as they do not rely on storing information from the training sets. Instead, they apply image transformations and filtering methods in memory. Also, VG, MD and ED require $0.018$, $0.023$ and $0.049$ secs, on average, to check if a single image is adversarial. Note that these runtimes are implementation specific and they may depend on the image dimensions. For instance, VG can be optimized by computing the softmax output of the original and the transformed image in parallel. %\IL{What is a typical frame rate, e.g. for self-driving car? It would be nice if we can state that VG can run at typical frame rates.} 
%Observe that as the dimensions of the input images increase, the runtime of VG increases slightly as well. This is expected as the JPEG compression/decompression time complexity is $O(n)$, where $n$ is the number of pixels \cite{chiou2017complexity}. Observe in the same table that MagNet and VG have similar execution times due to their similar structure but the KDE detector is faster than both as it does not require applying transformation to images. Nevertheless, as discussed earlier, its fast execution time is accompanied with poor performance on large-scale image domains; see Table \ref{tab:imagenet}. 
The employed single-image detectors are fast enough for real time applications, such as autonomous cars. For instance, the YOLO neural network \cite{redmon2016you} typically operates in autonomous driving applications at 55 frames per second (FPS) (or at 155 FPS for a small accuracy trade off) i.e., $55$ images are generated per second \cite{yurtsever2020survey}. Thus, if the car camera operates at $55$ FPS, then a new frame/image is generated every $0.018$ seconds. In other words, VG can be used to reason about trustworthiness of each frame while the entropy detector can be used every $0.049/0.018=2.78$ frames. %Nevertheless, this assumes that there is no other delay in the system which is hard to achieve in practice. 
%
Finally, applying majority vote is quite inexpensive. For instance, majority vote required on average $7.1\times 10^{-6}$ \text{secs}, $8.1\times 10^{-6}$ \text{secs}, $7.9\times 10^{-6}$ \text{secs}, and $1.1\times 10^{-5}$ \text{secs} for $T=3, 10, 30$ and $T=T_{\text{all}}$, respectively. We note that these runtimes ignore any computational burden incurred by e.g., object tracking algorithms that will generate sequences of images containing the same object of interest.



%As expected due to Proposition \ref{prop:betterPerf}, when the accuracy of the single-image detector on a video is greater than $50\%$, then then the performance of the time series detector increases as $T$ increases as well.




%Given a detection window of length $T$, each frame $x_t$ is classified as adversarial or clean using the time-series detector.
%

%First, using clean images from AdvNet, we train a YOLO v3 object detector that can detect stop, yield and speed limit 35 signs.
%Object detector (imperfect)
%Object tracking (perfect)
%Videos (single object)







%\IL{The graph in Fig 9 can be made smaller. Define what are red and blue lines.}

%\begin{figure}[t]
%  \centering
%  %\includegraphics[width=0.40\linewidth]{accuracyNN_vs_attacks_MNIST_CIFAR10.pdf}}
%    \includegraphics[width=1\linewidth]{ICCPS2021__VisionGuard/figures/ROC_B200_LISA_DRIVE.pdf}
%  \caption{ROC curve corresponding to VisionGuard equipped with brightness transformation with $\text{HSV}=200$ on stop traffic signs generated during the drive-by test for LISA CNN \cite{eykholt2018robust}; $\text{AUROC}=100\%$. The detection threshold $\tau=0.43$ yields $\text{TP rate}=100\%$ and $\text{FP rate}=0\%$.}
%   \label{fig:ROC2}
%\end{figure}
%\IL{In Fig 10, the graph can be made smaller.  Define what red and blue lines represent.}



%{\bf{Real-Time Computational Requirements:}} 



% T=3: 7.053323694177576e-06
% T=10: 8.14360541266364e-06
% T=30: 7.93096181508657e-06
% T= Inf: 1.0482684986011403e-05

%If e.g., VG requires $0.0179$ secs to reason about trustworthiness of an $32\times32\times3$ image, then it can be used to analyze $1 \text{sec}/0.0179 \text{secs}= 55.86$ frames within a second. $0.0179 \text{secs}* 55 \text{FPS}=4.4$ frames per second. In other words, it can be used to analyze every $12$-th frame assuming that the car camera operates at $55$ FPS.  %[to be updated..currently running simulations to receover the numbers..]}




%%% ENTROPY BASED DETECTOR%%
%\textcolor{red}{[THE NEXT TABLES REFER TO THE ENTROPY-BASED DETECTOR]}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}








